Emotions in Requirements Engineering: A Systematic Mapping Study

The purpose of requirements engineering (RE) is to make sure that the expectations and needs of the stakeholders of a software system are met. Emotional needs can be captured as emotional requirements that represent how the end user should feel when using the system. Differently from functional and quality (non-functional) requirements, emotional requirements have received relatively less attention from the RE community. This study is motivated by the need to explore and map the literature on emotional requirements. The study applies the systematic mapping study technique for surveying and analyzing the available literature to identify the most relevant publications on emotional requirements. We identified 34 publications that address a wide spectrum of practices concerned with engineering emotional requirements. The identified publications were analyzed with respect to the application domains, instruments used for eliciting and artefacts used for representing emotional requirements, and the state of the practice in emotion-related requirements engineering. This analysis serves to identify research gaps and research directions in engineering emotional requirements. To the best of the knowledge by the authors, no other similar study has been conducted on emotional requirements.

==> Background.tex <==
\section{Background:}
\label{sec:Background}

Talk about Requirement engineering 

discusses existing meta-studies in the area of emotions in requirements/software engineering. 

https://arxiv.org/pdf/1612.01556.pdf
Shiau, Wen-Lung, et al. "Cognition and emotion in the information systems field: a review of twenty-four years of literature." Enterprise Information Systems 16.6 (2022): 1992675.

%https://link.springer.com/content/pdf/10.1007/978-3-642-16324-1_1.pdf
https://doi.org/10.1016/j.infsof.2019.08.002

\textcolor{red}{ [MG - Probably, it is better to integrate this part within the first part of the introduction]}

A main factor in the success of any system is meeting its stakeholders' actual needs, which is usually used to derive the requirements for developing the system-to-be \cite{Softwareengineering8}. There is a general agreement that these requirements can be classified under functional and non-functional (quality) requirements [citation], where the first refers to the functionalities/services that the system should deliver, and the last refer to qualities that the system needs to satisfy while delivering the aforementioned services \cite{glinz2007non}. In this context, the success of a system is determined by satisfying both its functional and quality requirements, since functional requirements might not be useful without their necessarily related quality requirements \cite{chung2009non}.  Thus, an integrated analysis of both functional and quality requirements is essential to determine the system success and usefulness.

==> Tables/Domain_Category_Definitions.tex <==

\begin{table}[!htbp]
    \centering
  \caption{Domain categories of the selected publications}
\label{tab: Domain_Categories_Definitions}
    \resizebox{.80\textwidth}{!}{
    \begin{tabularx}{\textwidth}{c |X}
    \hline
  
    \textbf{ Domain category}\\ \hline
Smart-home\\ \hline
E-Learning\\ \hline
Well-being\\ \hline
Health-care\\ \hline
Mobile\\ \hline
Information System\\ \hline
Game development\\ \hline
Automated Vehicles\\ \hline
    \end{tabularx}
    }
\end{table}	

==> Tables/Pie_chart_stats.tex <==
\begin{table}[H]
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|p{3cm}|p{7cm}|p{2cm}|}
\hline
\textbf{Type} & \textbf{Primary publications} & \textbf{\# of publications} \\ \hline
Journal & P2,P3,P4,P8,P12,P19,P35,P36,P27 &  9 \\ \hline
Conference  & P11,P14,P16,P17,P18,P20,P23,P24,P29,
P34 & 14 \\ \hline
Book Chapter & P15, P21  & 2 \\ \hline
Workshop &P10,P13,P22,P25,P26,P30,P31, P32,P33  & 9 \\ \hline
Symposium & P5,P28 & 2 \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Proportions of articles by publication type}
\label{tab: Pie_chart_stats}
\end{table}

==> Tables/author2.tex <==
\begin{table}[!b]
%\vspace{-4mm}
\centering
%\begin{adjustbox}{width= 1\textwidth}
%\begin{tabularx}{>{\columncolor[HTML]{C0D9E6}}p{4cm}|p{6cm}|p{2cm}}
%\resizebox{.80\textwidth}{!}{%
%\begin{tabularx}{\textwidth}{X|p{6cm}|c}
\caption{Most active researchers in selected publications}
\label{tab: Most active researchers and their affiliations}
\begin{tabularx}{.48\textwidth}{X|X|p{3.5cm}}

\hline
\textbf{Author} &	\textbf{Ref.} &	\textbf{Affiliation}  \\ \hline
Tim Miller &	P3, P6, P8, P10, P15, P24 &	University of Melbourne, Australia \\ \hline
Sonja Pedell &	P3, P6, P10, P15, P30 &	Swinburne University of Technology, Australia \\ \hline
Antonette Mendoza &	P3, P6, P8, P10, P24 &	University of Melbourne, Australia \\ \hline
Leon Sterling &	P3, P6, P10, P15, P30 &	Swinburne University of Technology, Australia \\ \hline
John Grundy &	P4, P28, P33 &	Deakin University, Australia \& Monash University, Australia \\ \hline
Rachel Burrows &	P6, P8, P30 &	University of Melbourne, Australia \& Cambridge Science Park, UK \\ \hline
Alistair Sutcliffe &	P12, P13, P17 &	University of Manchester, UK \\ \hline
Kuldar Taveter &	P18, P19, P30 &	University of Tartu, Estonia \\ \hline
Ricardo Colomo-Palacios&	P2, P14,&	Universidad Carlos III de Madrid, Spain	\\ \hline
Simon André Scherr&	P1, P25	&Fraunhofer IESE, Kaiserslautern	Germany	\\ \hline
Patrick Mennig	&P1, P25 &	Fraunhofer IESE, Kaiserslautern	Germany	\\ \hline
Pedro Soto-Acosta&	P2, P14	&University of Murcia	Spain\\ \hline
Ángel García-Crespo&	P2, P14&	Universidad Carlos III de Madrid	Spain	\\ \hline
Frank Elberzhager&	P1 , P25 &	"University of Applied Sciences and Arts Northwestern, Switzerland \& Fraunhofer IESE, Kaiserslautern"	Germany	\\ \hline
Alen Keirnan &P3, P10 &	Swinburne University of Technology,	Australia\\ \hline
Antonio A. Lopez-Lorca &	P3, P10 &	Swinburne University of Technology	Australia	\\ \hline
Maheswaree Kissoon Curumsing &		P4 &Deakin University,Australia\\ \hline
Melanie Stade	&P1 &	University of Applied Sciences and Arts Northwestern,Switzerland\\ \hline
Gonçalo Miguéis	&	P5& FCT/UNL,Portugal\\ \hline
Danni Chang	&	P7& Nanyang Technological University,Singapore\\ \hline
Mohammadhossein Sherkat	&	P8 &	University of Melbourne,Australia\\ \hline
Cathy Grundy	&	P9 &	University of Brighton,Brighton\\ \hline
Aimée K. Bright&	P11 &	Northumbria University,UK\\ \hline
Sarah Thew	&	P12 &	Greater Manchester Academic Health Sciences Network,UK\\ \hline
Xueqing Zhao		&P16 &	East China University of Science and Technology,China\\ \hline
Ramón Martínez	&	P18 &	Universidad Politécnica de Cartagena, Spain\\ \hline
Kerli Mooses 	&	P19 &	University of Tartu, Estonia\\ \hline
Michael P. Craven&		P20& 	University of Nottingham, UK\\ \hline
Mary Zajicek &		P21 &	Oxford Brookes University, UK\\ \hline
Eric Jackson	&	P22 &	Tallinn University of Technology,Estonia\\ \hline
Takako Nakatani	&	P23 &	University of Tsukuba, Japan \\ \hline
Eman Alatawi	&	P24& 	University of Melbourne	, Australia\\ \hline
Zahra Shakeri Hossein Abad	&P26 	&University of Calgary, Canada\\ \hline
Emitza Guzman	&	P29 &	Technische Universität München, Germany\\ \hline
Meira Levy	&	P31 &	University of Haifa	, Israel\\ \hline
David Callele	&	P32& 	University of Saskatchewan, Canada\\ \hline
Nik Nailah Binti Abdullah	&	P33 &	Monash University, Malaysia\\ \hline
Andreas Gregoriades	&	P34 &	Cyprus University of Technology, Cyprus\\ \hline
S.Filzah Zulkifli	&	P27 &	Universiti Malaysia Sarawak, Malaysia\\ \hline
Cristina Casado-Lumbreras	&	P2 &	Universidad Complutense de Madrid, Spain\\ \hline
Niroshinie Fernando&		P4 &	Deakin University, Australia\\ \hline
João Araujo	&	P5 &	FCT/UNL, Portugal\\ \hline
Antonio Lopez-Lorca	&	P6 &	Semantic Web Company, Vienna, Austria\\ \hline
Yuexiang Huang	&	P7 &	Nanyang Technological University, Singapore\\ \hline
Lyn Pemberton	&	P9& 	University of Brighton,Brighton\\ \hline
Lynne Coventry	&	P11 &	Northumbria University, UK\\ \hline
Adrián Hernández-López	&	P14 &	Universidad Carlos III de Madrid, Spain\\ \hline
Wei Yu	&	P16 &	East China University of Science and Technology	 China\\ \hline
Francisco J. Moreno-Muro	&	P18& 	Universidad Politécnica de Cartagena, spain\\ \hline
Alexandra R. Lang&		P20 &	University of Nottingham, UK\\ \hline
Alex Norta	&	P22 	&Tallinn University of Technology, Estonia\\ \hline
Keita Sato	&	P23 &	DENSO Corporation	 Japan\\ \hline
Vincenzo Gervasi	&	P26 &	University of Pisa, Italy\\ \hline
Walid Maalej	&	P29 &	University of Hamburg, Germany\\ \hline
Eric Neufeld	&	P32 &	University of Saskatchewan, Canada\\ \hline
Maria Pampaka	&	P34 &	University of Manchester, UK\\ \hline
CW Shiang	&	P27 	&Universiti Malaysia Sarawak, Malaysia\\ \hline
Mohamed Abdelrazek	&	P4 &	Deakin University, Australia\\ \hline
Ana Moreira	&	P5 &	FCT/UNL, Portugal\\ \hline
Chun-Hsien Chen	&	P7&	Nanyang Technological University, Singapore\\ \hline
Richard Morris	&	P9 &	University of Brighton, Brighton\\ \hline
Xin Liang	&	P16 &	East China University of Science and Technology, China\\ \hline
Francisco J. Melero-Muñoz	&	P18 	Universidad Politécnica de Cartagena, Spain\\ \hline
Jennifer L. Martin	&	P20 &	The Institute of Mental Health, NIHR MindTech Healthcare Technology Co-operative, UK\\ \hline
Christian Kammler	&	P25 &	Fraunhofer IESE, Kaiserslautern, Germany\\ \hline
Didar Zowghi	&	P26 &	University of Technology Sydney, Australia\\ \hline
Kevin Schneider	&	P32 &	University of Saskatchewan,  Canada\\ \hline
Jennifer McIntosh	&	P33 &	Monash University, Australia\\ \hline
Michael Georgiades	&	P34 &	Primetel PLC, Limassol, Cyprus\\ \hline
N Jali	&	P27	& Universiti Malaysia Sarawak	 \\ \hline
Rajesh Vasa	&	P4 &	Deakin University, Australia\\ \hline
Li Pheng	&	P7 &	Nanyang Technological University, Singapore\\ \hline
Frank Vetere&		P15 &	University of Melbourne, Australia\\ \hline
María V. Bueno-Delgado	&	P18 &	Universidad Politécnica de Cartagena, Spain\\ \hline
Ken Barker		&P26 &	University of Calgary, Canada\\ \hline
Yen Chia How	&	P33 &	Clinical Research Center, Department of Cardiology, Hospital Queen Elizabeth II, Malaysia\\ \hline
M.A. Khairuddin	&	P27 &	Universiti Malaysia Sarawak,	 Malaysia\\ \hline
Norbert Seyff	&	P1 	&University of Applied Sciences and Arts Northwestern,Switzerland\\ \hline
Kon Mouzakis	&	P4 &	Deakin University, Australia\\ \hline
Steve Howard	&P15 &	University of Melbourne, Australia\\ \hline
Josefina Garrido-Lova	&	P18 &	Technical Research Centre of Furniture and Wood of the Region of Murcia (CETEM), Spain\\ \hline
Eliise Marie Taveter&		P30 &	University of Nottingham, UK\\ \hline
Sahrin Saharuddin	&	P33 &	Clinical Research Center, Department of Cardiology, Hospital Queen Elizabeth II,	 Malaysia\\ \hline
María Sánchez-Melero	&	P18 &	Technical Research Centre of Furniture and Wood of the Region of Murcia (CETEM), Spain\\ \hline
Koh Keng Tat	&	P33 &	Heart Failure Clinic, Pusat Jantung Sarawak, Malaysia\\ \hline
Eng ShinYe	&	P33 &	Heart Failure Clinic, Pusat Jantung Sarawak, Malaysia\\ \hline
Angie Julaina Anak Rastom	&	P33 &	Heart Failure Clinic, Pusat Jantung Sarawak, Malaysia\\ \hline
Noorma Liyana Othman	&	P33 &	Heart Failure Clinic, Pusat Jantung Sarawak, Malaysia\\ \hline


\end{tabularx}
%}
%\end{adjustbox}

%\vspace{-9mm}
\end{table}

==> Tables/requirementPhases.tex <==
\begin{table}[!htbp]
\resizebox{\textwidth}{!}{%
\begin{tabularx}{.80\textwidth}{X|p{4.5cm}|c}
\hline
\textbf{Artifact}                  & \textbf{Primary Studies} &  \# of studies \\ \hline
RE (in general)              &               P14       &          1   \\ \hline
Specification &    P8, P17   &  2  \\ \hline
Elicitation             &        P4, P10, P12, P3, P19, P20, P21, P27, P30, P31, P34, P35, P18   &   13 \\ \hline
Elicitation and Specification & P6, P15 ,P9, P11     &  4   \\ \hline
Elicitation and Prioritization  &         P1, P23      &   2        \\ \hline
Elicitation and Validation &      P5, P13             &      2       \\ \hline
Elicitation and Management &    P26                   &        1      \\ \hline
Elicitation and Evaluation&    P28, P25, P29, P22, P7 &         5     \\ \hline
Elicitation and Analysis  &           P32, P16         &      2       \\ \hline
Evolution and Management &    P2  &  1   \\ \hline
Elicitation, Validation and Evaluation & P27        &      1       \\ \hline
Elicitation, Modeling, and Analysis &    P33       &       1  \\ \hline


\end{tabularx}%
}
\caption{RE phases covered by selected studies}
\label{tab:RE phases covered by selected studies}
\end{table}
